Avoiding The Man on the Wire: Improving Tor's Security with Trust-Aware Path Selection

Tor users are vulnerable to deanonymization by an adversary that can observe some Tor relays or some parts of the network. We demonstrate that previous network-aware path-selection algorithms that propose to solve this problem are vulnerable to attacks across multiple Tor connections. We suggest that users use trust to choose the paths through Tor that are less likely to be observed, where trust is flexibly modeled as a probability distribution on the location of the user's adversaries, and we present the Trust-Aware Path Selection algorithm for Tor that helps users avoid traffic-analysis attacks while still choosing paths that could have been selected by many other users. We evaluate this algorithm in two settings using a high-level map of Internet routing: (i) users try to avoid a single global adversary that has an independent chance to control each Autonomous System organization, Internet Exchange Point organization, and Tor relay family, and (ii) users try to avoid deanonymization by any single country. We also examine the performance of Trust-Aware Path selection using the Shadow network simulator.

==> sections/trust.tex <==
\section{Obtaining and Propagating Trust}
This section should describe how we expect trust information to be obtained, processed, and
distributed among relays and users.

In order to use trust to make decisions about route selection, clients
require either adequate trust information themselves or the results of
trust-aware routing algorithms performed on their behalf.

For a widely used trust-aware Tor supporting diversely trusting
populations we may need to consider propagating trust via directory
systems with controls on what trust information is distributed to whom
and controls on what the directory servers know about what they are
distributing. Even more ambitiously, it is conceivable that instead of
circuit choices being entirely source routed, clients can safely offload
some route selection decisions to trusted relays. Less ambitiously,
we can simply ask what basic information needs to be passed to clients
to support trust-aware route selection as we have been describing in
this paper.

We will assume that default relay trust information is distributed via the
same directory and distribution system that Tor currently uses to
distribute information about relays and their state. This depends
largely on information about relays that directory authorities use for
creating and distributing network status information already. 

Default link trust information is primarily based on information
not currently gathered by Tor directory authorities. This information
could be gathered by relays themselves and signed. It would then
make sense to have this distributed via directory authorities.

We assume clients that are not using default trust information will
have obtained it separately in some way. For example, workstation
clients may have received it over a private LAN from whatever
authority provides them their trust information. Mobile clients can
obtain trust information either via an offline mechanism or when
locally connected to a protected private network, for example, prior
to going away on a trip or periodically for telecommuting.

Returning to the default trust case, what information do clients need
to do trust-aware route selection? On the source end of any circuit
they will just need the scores for guard choices according to their
IP cluster. In other words, this part of the trust determination should
effectively have already been made for them and will be captured in
a small set numbers. On the destination end, things are a bit more
complex. 

%%% Local Variables: 
%%% mode: latex 
%%% TeX-master: "../paper"
%%% End:          

